Robust Learning Through Cross-Task Consistency

Visual perception entails solving a wide set of tasks, e.g., object detection, depth estimation, etc. The predictions made for multiple tasks from the same image are not independent, and therefore, are expected to be consistent. We propose a broadly applicable and fully computational method for augmenting learning with Cross-Task Consistency. The proposed formulation is based on inference-path invariance over a graph of arbitrary tasks. We observe that learning with cross-task consistency leads to more accurate predictions and better generalization to out-of-distribution inputs. This framework also leads to an informative unsupervised quantity, called Consistency Energy, based on measuring the intrinsic consistency of the system. Consistency Energy correlates well with the supervised error (r=0.67), thus it can be employed as an unsupervised confidence metric as well as for detection of out-of-distribution inputs (ROC-AUC=0.95). The evaluations are performed on multiple datasets, including Taskonomy, Replica, CocoDoom, and ApolloScape, and they benchmark cross-task consistency versus various baselines including conventional multi-task learning, cycle consistency, and analytical consistency.

==> tables/REPLICA/depth2ALL.tex <==
\addtolength{\tabcolsep}{-2.5pt}\begin{tabular}{|c|cc|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{
\backslashbox{Method}{\hspace{-0mm}\vspace{0mm}\tiny{\textbf{Depth} $\rightarrow$ X}}
}} & \multicolumn{2}{c|}{\scriptsize{Perceptual ({$\downarrow$})}} & \multicolumn{1}{c|}{Direct}\\
& \multicolumn{1}{c}{Normals} & \multicolumn{1}{c|}{reShading} & L1 \tiny{$(\downarrow)$} \\
\hline
\hline
Blind Guess            &         22.23   &         19.94   &         4.81   \\
Taskonomy                 &         18.06   &         15.39   &         3.72   \\
Multitask                 &         15.30   &         16.14   &         2.44   \\
GeoNet (Orig.) &         13.88   &         14.03   &         4.01   \\
Baseline (L1 UNet)           &         10.47   &         12.99   &         1.99   \\
GeoNet (Impr.) &         10.47   &         12.75   &         1.83   \\
\textbf{X-Task Consistency}      & \textbf{7.01} & \textbf{11.21} & \textbf{1.63} \\
\hline
\end{tabular}
\addtolength{\tabcolsep}{2.5pt}

% \addtolength{\tabcolsep}{-2.5pt}\begin{tabular}{|c|cc|c|}
% \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{
% \backslashbox{Method}{\vspace{-1mm}\tiny{\textbf{Depth} $\rightarrow$ X}}
% }} & \multicolumn{2}{c|}{\scriptsize{Perceptual Error (L1 \tiny{$\downarrow$})}} & \multicolumn{1}{c|}{Error}\\
% & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c|}{reShading} & L1 \tiny{$(\downarrow)$} \\
% \hline
% \hline
% Baseline (UNet)           &         10.47   &         12.99   &         1.99   \\
% Constant Pred.            &         22.23   &         19.94   &         4.81   \\
% GeoNet  (Impr.) &         10.47   &         12.75   &         1.83   \\
% GeoNet (Orig.) &         13.88   &         14.03   &         4.01   \\
% Multitask                 &         15.30   &         16.14   &         2.44   \\
% Taskonomy                 &         18.06   &         15.39   &         3.72   \\
% \textbf{Consistency}      & \textbf{7.01} & \textbf{11.21} & \textbf{1.63} \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2.5pt}

% \addtolength{\tabcolsep}{-2.5pt}\begin{tabular}{|c|c|cc|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Depth} $\rightarrow$}& \multicolumn{1}{c|}{Error}& \multicolumn{2}{c|}{\scriptsize{Perceptual Error (L1 \tiny{$\downarrow$})}} \\
% \multicolumn{1}{|c|}{Method} & L1 \tiny{$(\downarrow)$} & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c|}{reShading} \\
% \hline
% \hline
% Baseline (UNet)           &         1.99   &         10.47   &         12.99   \\
% Constant Pred.            &         4.81   &         22.23   &         19.94   \\
% GeoNet~\cite{Geonet18}  (Impr.) &         1.83   &         10.47   &         12.75   \\
% GeoNet~\cite{Geonet18} (Orig.) &         4.01   &         13.88   &         14.03   \\
% Multitask                 &         2.44   &         15.30   &         16.14   \\
% Taskonomy                 &         3.72   &         18.06   &         15.39   \\
% \textbf{Consistency}      & \textbf{1.63} & \textbf{7.01} & \textbf{11.21} \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2.5pt}

==> tables/REPLICA/normal2ALL.tex <==
\addtolength{\tabcolsep}{-2.5pt}\begin{tabular}{|c|cc|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{
\backslashbox{Method}{\hspace{-0.0mm}\vspace{0mm}\tiny{\textbf{Normals} $\rightarrow$ X}}
}} & \multicolumn{2}{c|}{{Perceptual ({$\downarrow$})}} & \multicolumn{1}{c|}{Direct}\\
  & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c|}{reShading} & L1 \tiny{$(\downarrow)$} \\
\hline
\hline
GeoNet (Orig.) &         6.23   &         19.34    &         7.48   \\
Cycle Consistency         &         5.65   &         22.39    &         7.13      \\
Multitask                 &         5.58   &         22.11    &         6.03   \\
Prcpt. Loss (Random)      &         4.88   &         15.34    &         4.99   \\
Blind Guess            &         4.75   &         33.31    &         16.02   \\
Baseline (UNet)           &         4.69   &         13.15    &         4.96  \\
GeoNet (Impr.) &         4.62   &         12.79   & \textbf{4.70} \\
Pix2Pix    &         4.52   &         19.03    &         7.70   \\
\textbf{X-Task Consistency}      & \textbf{2.07} &         9.99   & \textbf{4.80}  \\
\hline
0.25\% Data: Baseline          &         5.65   &         21.76    &         7.61   \\
\textbf{0.25\% Data: Consistency}    & \textbf{2.41} & \textbf{12.26} & \textbf{7.28} \\
\hline
\end{tabular}
\addtolength{\tabcolsep}{2.5pt}
% \addtolength{\tabcolsep}{-2.5pt}\begin{tabular}{|c|c|cc|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Normals} $\rightarrow$}& \multicolumn{1}{c|}{Error}& \multicolumn{2}{c|}{{Perceptual Error (L1 \tiny{$\downarrow$})}} \\
% \multicolumn{1}{|c|}{Method} & L1 \tiny{$(\downarrow)$} & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c|}{reShading} \\
% \hline
% \hline
% Baseline (UNet)           &         4.96   &         4.69   &         13.15   \\
% Constant Pred.            &         16.02   &         4.75   &         33.31   \\
% Cycle Consistency         &         7.13   &         5.65   &         22.39   \\
% GeoNet~\cite{Geonet18}  (Impr.) & \textbf{4.70} &         4.62   &         12.79   \\
% GeoNet~\cite{Geonet18} (Orig.) &         7.48   &         6.23   &         19.34   \\
% Multitask                 &         6.03   &         5.58   &         22.11   \\
% Pix2Pix~\cite{pix2pix}    &         7.70   &         4.52   &         19.03   \\
% Prcpt. Loss (Random)      &         4.99   &         4.88   &         15.34   \\
% \textbf{Consistency}      & \textbf{4.80}  & \textbf{2.07} &         9.99   \\
% \hline
% 0.25\% Data: Baseline           &         7.61   &         5.65   &         21.76   \\
% \textbf{0.25\% Data: Consistency}      & \textbf{7.28} & \textbf{2.41} & \textbf{12.26} \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2.5pt}


==> tables/REPLICA/reshading2ALL.tex <==

\addtolength{\tabcolsep}{-2.5pt}\begin{tabularx}{\textwidth}{|c|cc|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{
\backslashbox{Method}{\hspace{-2.7mm}\vspace{0mm}\tiny{\textbf{reShading} $\rightarrow$ X}}
}}
& \multicolumn{2}{c|}{Perceptual $(\downarrow)$} & \multicolumn{1}{c|}{Direct}\\
%  & \multicolumn{1}{c}{reShading $\rightarrow$} & \multicolumn{1}{c|}{reShading $\rightarrow$} & $(\downarrow)$ \\
 & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c|}{Depth} & L1 \tiny{$(\downarrow)$} \\
\hline
\hline
Blind Guess            &         15.74   &         5.14  &         16.45    \\
Taskonomy                 &         8.70   &         3.85   &         11.43   \\
Multitask                 &         7.24   &         3.36   &         10.32   \\
Baseline (L1 UNet)           &         6.90   &         2.74   & \textbf{9.55}  \\
\textbf{X-Task Consistency}      & \textbf{5.50} & \textbf{1.96}   & \textbf{9.22} \\
\hline
\end{tabularx}
\addtolength{\tabcolsep}{2.5pt}


% \addtolength{\tabcolsep}{-2.5pt}\begin{tabular}{|c|cc|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{reShading} $\rightarrow$}& \multicolumn{2}{c|}{Perceptual Error (L1 \tiny{$\downarrow$})} & \multicolumn{1}{c|}{Error}\\
% \multicolumn{1}{|c|}{Method} & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c|}{Depth} & L1 \tiny{$(\downarrow)$} \\
% \hline
% \hline
% Baseline (UNet)           &         6.90   &         2.74   & \textbf{9.55}  \\
% Constant Pred.            &         15.74   &         5.14  &         16.45    \\
% Multitask                 &         7.24   &         3.36   &         10.32   \\
% Taskonomy                 &         8.70   &         3.85   &         11.43   \\
% \textbf{Consistency}      & \textbf{5.50} & \textbf{1.96}   & \textbf{9.22} \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2.5pt}


% \addtolength{\tabcolsep}{-2.5pt}\begin{tabular}{|c|c|cc|}
% \hline
% \multicolumn{1}{|c|}{\textbf{reShading} $\rightarrow$}& \multicolumn{1}{c|}{Error}& \multicolumn{2}{c|}{Perceptual Error (L1 \tiny{$\downarrow$})} \\
% \multicolumn{1}{|c|}{Method} & L1 \tiny{$(\downarrow)$} & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c|}{Depth} \\
% \hline
% \hline
% Baseline (UNet)           & \textbf{9.55}  &         6.90   &         2.74   \\
% Constant Pred.            &         16.45   &         15.74   &         5.14   \\
% Multitask                 &         10.32   &         7.24   &         3.36   \\
% Taskonomy                 &         11.43   &         8.70   &         3.85   \\
% \textbf{Consistency}      & \textbf{9.22} & \textbf{5.50} & \textbf{1.96} \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2.5pt}


==> tables/TASKONOMY_TEST/depth2ALL.tex <==
\addtolength{\tabcolsep}{-2pt}\begin{tabular}{|c|cccc|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{
\backslashbox{Method}{\hspace{-0mm}\vspace{0mm}\tiny{\textbf{Depth} $\rightarrow$ X}}
}} & \multicolumn{4}{c|}{Perceptual $(\downarrow)$} & \multicolumn{1}{c|}{Direct}\\
 & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c}{reShading} & \multicolumn{1}{c}{Curvature} & \multicolumn{1}{c|}{Edges (2D)} & L1 $(\downarrow)$ \\
\hline
\hline
Baseline (L1 UNet)           &         13.62   &         15.68   &         7.31   &         12.61   & \textbf{2.27}  \\
Blind Guess            &         22.37   &         27.27   &         7.96   &         12.77   &         7.07    \\
GeoNet  (Impr.) &         13.77   &         15.76   &         7.52   &         12.67   & \textbf{2.26}  \\
GeoNet (Orig.)  &         15.44   &         18.73   &         4.03   &         10.78  &         4.07   \\
Multitask                 &         17.18   &         19.55   &         7.54   &         13.67  &         2.81    \\
Taskonomy                 &         18.82   &         20.83   &         6.65   &         14.10  &         4.55    \\
\textbf{X-Task Consistency}      & \textbf{9.46} & \textbf{12.66} & \textbf{3.61} & \textbf{9.82}  & \textbf{2.29}  \\
\hline
\end{tabular}
\addtolength{\tabcolsep}{2pt}

% \addtolength{\tabcolsep}{-2pt}\begin{tabular}{|c|c|cccc|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Depth} $\rightarrow$}& \multicolumn{1}{c|}{Error $(\downarrow)$}& \multicolumn{4}{c|}{Perceptual Error (L1) $(\downarrow)$} \\
% \multicolumn{1}{|c|}{Method} & L1 & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c}{reShading} & \multicolumn{1}{c}{Curvature} & \multicolumn{1}{c|}{Edges (2D)} \\
% \hline
% \hline
% Baseline (UNet)           & \textbf{2.27}  &         13.62   &         15.68   &         7.31   &         12.61   \\
% Constant Pred.            &         7.07   &         22.37   &         27.27   &         7.96   &         12.77   \\
% GeoNet~\cite{Geonet18}  (Impr.) & \textbf{2.26} &         13.77   &         15.76   &         7.52   &         12.67   \\
% GeoNet~\cite{Geonet18} (Orig.) &         4.07   &         15.44   &         18.73   &         4.03   &         10.78   \\
% Multitask                 &         2.81   &         17.18   &         19.55   &         7.54   &         13.67   \\
% Taskonomy                 &         4.55   &         18.82   &         20.83   &         6.65   &         14.10   \\
% \textbf{Consistency}      & \textbf{2.29}  & \textbf{9.46} & \textbf{12.66} & \textbf{3.61} & \textbf{9.82} \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2pt}

==> tables/TASKONOMY_TEST/normal2ALL.tex <==
\addtolength{\tabcolsep}{-2pt}\begin{tabular}{|c|cccc|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{
\backslashbox{Method}{\hspace{-0.0mm}\vspace{0mm}\tiny{\textbf{Normals} $\rightarrow$ X}}
}}& \multicolumn{4}{c|}{Perceptual $(\downarrow)$} & \multicolumn{1}{c|}{Direct}\\
 & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c}{reShading} & \multicolumn{1}{c}{Curvature} & \multicolumn{1}{c|}{Edges (2D)} & L1 $(\downarrow)$ \\
\hline
\hline
Cycle Consistency         &         8.81   &         30.33   &         3.84   &         10.26  &         8.68    \\
Multitask                 &         8.78   &         27.32   &         3.65   &         10.16   &         7.07    \\
Prcpt. Loss (Random)      &         8.59   &         23.98   &         3.41   &         10.01   &         6.17   \\
GeoNet  (Impr.) &         8.18   &         20.84   &         3.40   &         9.99  & \textbf{5.91}  \\
Pix2Pix    &         8.12   &         26.23   &         3.83   &         10.33   &         9.40   \\
Baseline (L1 UNet)           &         8.17   &         20.94   &         3.41   &         9.98   & \textbf{5.95}  \\
GeoNet (Orig.)  &         7.71   &         27.35   & \textbf{3.32}  & \textbf{9.09} &         9.58  \\
% Prcpt. Loss (ImageNet)    &         6.86   &         17.36   &         3.36   &         9.63    &         6.06   \\
Blind Guess         &         7.39   &         38.11   &         3.91   &        12.05  &         17.77   \\
\textbf{X-Task Consistency}      & \textbf{4.32} & \textbf{12.15} & \textbf{3.29} &         9.50   &         6.08   \\
\hline
0.25\% Data: Baseline           &         8.86   &         26.91   &         3.78   &         10.31  & \textbf{8.17}  \\
\textbf{0.25\% Data: Consistency}      & \textbf{5.07} & \textbf{15.96} & \textbf{3.74} & \textbf{9.93} &         9.19   \\
\hline
\end{tabular}
\addtolength{\tabcolsep}{2pt}


% \addtolength{\tabcolsep}{-2pt}\begin{tabular}{|c|cccc|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Normals} $\rightarrow$}& \multicolumn{4}{c|}{Perceptual Error (L1) $(\downarrow)$} & \multicolumn{1}{c|}{Error $(\downarrow)$}\\
% \multicolumn{1}{|c|}{Method} & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c}{reShading} & \multicolumn{1}{c}{Curvature} & \multicolumn{1}{c|}{Edges (2D)} & L1  \\
% \hline
% \hline
% Baseline (UNet)           &         8.17   &         20.94   &         3.41   &         9.98   & \textbf{5.95}  \\
% Cycle Consistency         &         8.81   &         30.33   &         3.84   &         10.26  &         8.68    \\
% GeoNet~\cite{Geonet18}  (Impr.) &         8.18   &         20.84   &         3.40   &         9.99  & \textbf{5.91}  \\
% GeoNet~\cite{Geonet18} (Orig.)  &         7.71   &         27.35   & \textbf{3.32}  & \textbf{9.09} &         9.58  \\
% Multitask                 &         8.78   &         27.32   &         3.65   &         10.16   &         7.07    \\
% Pix2Pix~\cite{pix2pix}    &         8.12   &         26.23   &         3.83   &         10.33   &         9.40   \\
% % Prcpt. Loss (ImageNet)    &         6.86   &         17.36   &         3.36   &         9.63    &         6.06   \\
% Prcpt. Loss (Random)      &         8.59   &         23.98   &         3.41   &         10.01   &         6.17   \\
% \textbf{Consistency}      & \textbf{4.32} & \textbf{12.15} & \textbf{3.29} &         9.50   &         6.08   \\
% \hline
% 0.25\% Data: Baseline           &         8.86   &         26.91   &         3.78   &         10.31  & \textbf{8.17}  \\
% \textbf{0.25\% Data: Consistency}      & \textbf{5.07} & \textbf{15.96} & \textbf{3.74} & \textbf{9.93} &         9.19   \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2pt}


% \addtolength{\tabcolsep}{-2pt}\begin{tabular}{|c|c|cccc|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Normals} $\rightarrow$}& \multicolumn{1}{c|}{Error $(\downarrow)$}& \multicolumn{4}{c|}{Perceptual Error (L1) $(\downarrow)$} \\
% \multicolumn{1}{|c|}{Method} & L1 & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c}{reShading} & \multicolumn{1}{c}{Curvature} & \multicolumn{1}{c|}{Edges (2D)} \\
% \hline
% \hline
% Baseline (UNet)           & \textbf{5.95}  &         8.17   &         20.94   &         3.41   &         9.98   \\
% Cycle Consistency         &         8.68   &         8.81   &         30.33   &         3.84   &         10.26   \\
% GeoNet~\cite{Geonet18}  (Impr.) & \textbf{5.91} &         8.18   &         20.84   &         3.40   &         9.99   \\
% GeoNet~\cite{Geonet18} (Orig.) &         9.58   &         7.71   &         27.35   & \textbf{3.32}  & \textbf{9.09} \\
% Multitask                 &         7.07   &         8.78   &         27.32   &         3.65   &         10.16   \\
% Pix2Pix~\cite{pix2pix}    &         9.40   &         8.12   &         26.23   &         3.83   &         10.33   \\
% Prcpt. Loss (ImageNet)    &         6.06   &         6.86   &         17.36   &         3.36   &         9.63   \\
% Prcpt. Loss (Random)      &         6.17   &         8.59   &         23.98   &         3.41   &         10.01   \\
% \textbf{Consistency}      &         6.08   & \textbf{4.32} & \textbf{12.15} & \textbf{3.29} &         9.50   \\
% \hline
% 0.25\% Data: Baseline           & \textbf{8.17} &         8.86   &         26.91   &         3.78   &         10.31   \\
% \textbf{0.25\% Data: Consistency}      &         9.19   & \textbf{5.07} & \textbf{15.96} & \textbf{3.74} & \textbf{9.93} \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2pt}

==> tables/TASKONOMY_TEST/reshading2ALL.tex <==
\addtolength{\tabcolsep}{-2pt}\begin{tabular}{|c|cccc|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{
\backslashbox{Method}{\hspace{-2.7mm}\vspace{0mm}\tiny{\textbf{reShading} $\rightarrow$ X}}
}} & \multicolumn{4}{c|}{Perceptual $(\downarrow)$} & \multicolumn{1}{c|}{Direct}\\
 & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c}{Curvature} & \multicolumn{1}{c|}{Edges (2D)} & L1 $(\downarrow)$ \\
\hline
\hline
Blind Guess            &         19.96   &         7.14   &         3.53   &         12.62  &         24.85    \\
Taskonomy                 &         11.72   &         4.69   &         3.54   &         11.19  &         16.58    \\
~\hspace{1.5mm}Baseline (L1 UNet)\hspace{1.5mm}~&         9.58   &         3.38   &         3.78   &         10.85   & \textbf{10.45} \\
Multitask                 &         9.19   &         3.54   &         3.56   &         10.75   &         11.61   \\
\textbf{X-Task Consistency}      & \textbf{7.13} & \textbf{2.51} & \textbf{3.28} & \textbf{9.38} & \textbf{10.52}  \\
\hline
\end{tabular}
\addtolength{\tabcolsep}{2pt}

% \addtolength{\tabcolsep}{-1pt}\begin{tabular}{|c|cccc|c|}
% \hline
% \multicolumn{1}{|c|}{\textbf{reShading} $\rightarrow$}& \multicolumn{4}{c|}{Perceptual Error (L1) $(\downarrow)$} & \multicolumn{1}{c|}{Error $(\downarrow)$}\\
% \multicolumn{1}{|c|}{Method} & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c}{Curvature} & \multicolumn{1}{c|}{Edges (2D)} & L1 \\
% \hline
% \hline
% ~\hspace{1.5mm}Baseline (UNet)\hspace{1.5mm}~&         9.58   &         3.38   &         3.78   &         10.85   & \textbf{10.45} \\
% Constant Pred.            &         19.96   &         7.14   &         3.53   &         12.62  &         24.85    \\
% Multitask                 &         9.19   &         3.54   &         3.56   &         10.75   &         11.61   \\
% Taskonomy                 &         11.72   &         4.69   &         3.54   &         11.19  &         16.58    \\
% \textbf{Consistency}      & \textbf{7.13} & \textbf{2.51} & \textbf{3.28} & \textbf{9.38} & \textbf{10.52}  \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2pt}


% \addtolength{\tabcolsep}{-2pt}\begin{tabular}{|c|c|cccc|}
% \hline
% \multicolumn{1}{|c|}{\textbf{reShading} $\rightarrow$}& \multicolumn{1}{c|}{Error $(\downarrow)$}& \multicolumn{4}{c|}{Perceptual Error (L1) $(\downarrow)$} \\
% \multicolumn{1}{|c|}{Method} & L1 & \multicolumn{1}{c}{Normals} & \multicolumn{1}{c}{Depth} & \multicolumn{1}{c}{Curvature} & \multicolumn{1}{c|}{Edges (2D)} \\
% \hline
% \hline
% Baseline (UNet)           & \textbf{10.45} &         9.58   &         3.38   &         3.78   &         10.85   \\
% Constant Pred.            &         24.85   &         19.96   &         7.14   &         3.53   &         12.62   \\
% Multitask                 &         11.61   &         9.19   &         3.54   &         3.56   &         10.75   \\
% Taskonomy                 &         16.58   &         11.72   &         4.69   &         3.54   &         11.19   \\
% \textbf{Consistency}      & \textbf{10.52}  & \textbf{7.13} & \textbf{2.51} & \textbf{3.28} & \textbf{9.38} \\
% \hline
% \end{tabular}
% \addtolength{\tabcolsep}{2pt}

==> tables/joint_tables2.tex <==
\addtolength{\tabcolsep}{-5pt}\begin{tabular}{|c|cc|c|cc|c|cc|c|cccc|c|cccc|c|cccc|c|c|}
    \hline
    \multicolumn{1}{|c|}{\multirow{4}{*}{
    \backslashbox{~~Method}{\hspace{-0mm}\vspace{4.1mm}{~~~~~~~~~~Setup~~}}
    }} 
    & \multicolumn{9}{c|}{Replica Dataset} 
    & \multicolumn{16}{c|}{Taskonomy Dataset} \\
    \cline{2-26}
    & \multicolumn{3}{c|}{\textbf{Depth} } 
    & \multicolumn{3}{c|}{\textbf{Normals} } 
    & \multicolumn{3}{c|}{\textbf{reShading} } 
    & \multicolumn{5}{c|}{\textbf{Depth} } 
    & \multicolumn{5}{c|}{\textbf{Normals} } 
    & \multicolumn{5}{c|}{\textbf{reShading} } 
    & \multicolumn{1}{c|}{\textbf{Semantic Segm.}} \\
    % \cline{2-26}
    % &
    & \multicolumn{2}{c|}{Perceptual Err.} & \multicolumn{1}{c|}{Direct}
    & \multicolumn{2}{c|}{Perceptual Err.} & \multicolumn{1}{c|}{Direct}
    & \multicolumn{2}{c|}{Perceptual Err.} & \multicolumn{1}{c|}{Direct}
    & \multicolumn{4}{c|}{Perceptual Err.} & \multicolumn{1}{c|}{Direct}
    & \multicolumn{4}{c|}{Perceptual Err.} & \multicolumn{1}{c|}{Direct}
    & \multicolumn{4}{c|}{Perceptual Err.} & \multicolumn{1}{c|}{Direct}
    & \multicolumn{1}{c|}{Direct} \\
    & Norm. & reShade  & $l_1$ 
    & Depth & reShade  & $l_1$ 
    & Norm. & Depth  & $l_1$ 
    & Norm. & reShade & Curv. & \multicolumn{1}{c|}{Edge(2D)} & $l_1$  
    & Depth & reShade & Curv. & \multicolumn{1}{c|}{Edge(2D)} & $l_1$  
    & Norm. & Depth & Curv. & \multicolumn{1}{c|}{Edge(2D)} & $l_1$   
    & X-Entropy \\
    \hline
    \hline
    Blind Guess    &
            22.23  &         19.94  &         4.81   &
            4.75   &         33.31  &         16.02  & 
            15.74  &         5.14   &         16.45  & 
            22.37  &         27.27  &         7.96   &         12.77  &         7.07   &
            7.39   &         38.11  &         3.91   &         12.05  &         17.77  &
            19.96  &         7.14   &         3.53   &         12.62  &         24.85  &
            -  \\
    Taskonomy Networks     &
            18.06  &         15.39  &         3.72   & 
            3.73   &         11.07  &         6.55   & 
            8.70   &         3.85   &         11.43  & 
            18.82  &         20.83  &         6.65   &         14.10  &         4.55   &
            7.19   &         22.68  &         3.68   &         10.70  &         7.54   & 
            11.72  &         4.69   &         3.54   &         11.19  &         16.58  &
            -  \\
    Multi-Task      &
            15.30  &         16.14  &         2.44   & 
            5.58   &         22.11  &         6.03   & 
            7.24   &         3.36   &         10.32  & 
            17.18  &         19.55  &         7.54   &         13.67  &         2.81   &
            8.78   &         27.32  &         3.65   &         10.16  &         7.07   &
            9.19   &         3.54   &         3.56   &         10.75  &         11.61  &
            -  \\
    Cycle Consistency         &
            -      &         -      &         -      & 
            5.65   &         22.39  &         7.13   & 
            -      &         -      &         -      & 
            -      &         -      &         -      &         -      &         -      & 
            8.81   &         30.33  &         3.84   &         10.26  &         8.68   & 
            -      &         -      &         -      &         -      &         -      & 
            -  \\
    GeoNet  (original)                 &
            13.88  &         14.03  &          4.01  & 
            6.23   &         19.34  &          7.48  & 
            \na    &         \na    &          \na   &
            15.44  &         18.73  &          4.03  &         10.78  &        4.07   & 
            7.71   &         27.35  &  \textbf{3.32} &  \textbf{9.09} &        9.58   & 
            \na    &         \na    &          \na   &         \na    &        \na    &
            \na    \\
    Baseline Perceptual Loss            &
            -      &         -      &         -      & 
            4.88   &         15.34  &         4.99   & 
            -      &         -      &         -      & 
            -      &         -      &         -      &         -      &         -      & 
            8.59   &         23.98  &         3.41   &         10.01  &         6.17   & 
            -      &         -      &         -      &         -      &         -      & 
            -  \\
    Pix2Pix                         &
            -      &         -      &         -      & 
            4.52   &         19.03  &         7.70   & 
            -      &         -      &         -      & 
            -      &         -      &         -      &         -      &         -      & 
            8.12   &         26.23  &         3.83   &         10.33  &         9.40   & 
            -      &         -      &         -      &         -      &         -      & 
            -  \\
    Baseline UNet ($l_1$)              &
            10.47  &         12.99  &          1.99  & 
            4.69   &         13.15  &          4.96  & 
            6.90   &         2.74   &  \textbf{9.55} & 
            13.62  &         15.68  &          7.31  &         12.61  & \textbf{2.27}  &
            8.17   &         20.94  &          3.41  &         9.98   & \textbf{5.95}  &
            9.58   &         3.38   &          3.78  &         10.85  & \textbf{10.45} &
            0.246  \\
    GeoNet  (updated)                 &
            10.47  &         12.75  &          1.83  & 
            4.62   &         12.79  &  \textbf{4.70} & 
            \na    &         \na    &          \na   &
            13.77  &         15.76  &          7.52  &         12.67  & \textbf{2.26}  & 
            8.18   &         20.84  &          3.40  &         9.99   & \textbf{5.91}  & 
            \na    &         \na    &          \na   &         \na    &         \na    &
            \na    \\
    \textbf{X-Task Consistency}     &
            \textbf{7.01} & \textbf{11.21} & \textbf{1.63} & 
            \textbf{2.07} & \textbf{9.99}  & \textbf{4.80} & 
            \textbf{5.50} & \textbf{1.96}  & \textbf{9.22} & 
            \textbf{9.46} & \textbf{12.66} & \textbf{3.61} & \textbf{9.82} & \textbf{2.29}  &
            \textbf{4.32} & \textbf{12.15} & \textbf{3.29} &         9.50  &         6.08   &
            \textbf{7.13} & \textbf{2.51}  & \textbf{3.28} & \textbf{9.38} & \textbf{10.52} &
            \textbf{0.237}  \\
    \hline
    \hline
    0.25\% Data: Baseline           &
            -      &         -      &         -     & 
            5.65   &         21.76  &         7.61  & 
            -      &         -      &         -     & 
            -      &         -      &         -     &         -      &         -      & 
            8.86   &         26.91  &         3.78  &         10.31  & \textbf{8.17}  &
            -      &         -      &         -     &         -      &         -      & 
            -  \\
    \textbf{0.25\% Data: Consistency}        &
            -      &         -      &         -     & 
            \textbf{2.41} & \textbf{12.26} & \textbf{7.28} & 
            -      &         -      &         -     & 
            -      &         -      &         -     &         -      &         -      & 
            \textbf{5.07} & \textbf{15.96} & \textbf{3.74} & \textbf{9.93} &         9.19  &
            -      &         -      &         -     &         -      &         -      & 
            -  \\
    \hline

    % Multi-Task                 &         8.78   &         27.32   &         3.65   &         10.16   &         7.07    \\
    % Baseline Perceptual Loss      &         8.59   &         23.98   &         3.41   &         10.01   &         6.17   \\
    % GeoNet  (updated) &         8.18   &         20.84   &         3.40   &         9.99  & \textbf{5.91}  \\
    % Pix2Pix    &         8.12   &         26.23   &         3.83   &         10.33   &         9.40   \\
    % Baseline UNet ($l_1$)           &         8.17   &         20.94   &         3.41   &         9.98   & \textbf{5.95}  \\
    % GeoNet (original)  &         7.71   &         27.35   & \textbf{3.32}  & \textbf{9.09} &         9.58  \\
    % % Perceptual Loss (ImageNet)    &         6.86   &         17.36   &         3.36   &         9.63    &         6.06   \\
    % Blind Guess         &         7.39   &         38.11   &         3.91   &        12.05  &         17.77   \\
    % \textbf{X-Task Consistency}      & \textbf{4.32} & \textbf{12.15} & \textbf{3.29} &         9.50   &         6.08   \\
    % \hline
    % 0.25\% Data: Baseline           &         8.86   &         26.91   &         3.78   &         10.31  & \textbf{8.17}  \\
    % \textbf{0.25\% Data: Consistency}      & \textbf{5.07} & \textbf{15.96} & \textbf{3.74} & \textbf{9.93} &         9.19   \\
    % \hline
    \end{tabular}
    \addtolength{\tabcolsep}{5pt}
    
    
